BLT: Bidirectional Layout Transformer for Controllable Layout Generation

Creating visual layouts is a critical step in graphic design. Automatic generation of such layouts is essential for scalable and diverse visual designs. To advance conditional layout generation, we introduce BLT, a bidirectional layout transformer. BLT differs from previous work on transformers in adopting non-autoregressive transformers. In training, BLT learns to predict the masked attributes by attending to surrounding attributes in two directions. During inference, BLT first generates a draft layout from the input and then iteratively refines it into a high-quality layout by masking out low-confident attributes. The masks generated in both training and inference are controlled by a new hierarchical sampling policy. We verify the proposed model on six benchmarks of diverse design tasks. Experimental results demonstrate two benefits compared to the state-of-the-art layout transformer models. First, our model empowers layout transformers to fulfill controllable layout generation. Second, it achieves up to 10x speedup in generating a layout at inference time than the layout transformer baseline. Code is released at https://shawnkx.github.io/blt.

==> tables/conditional_merge.tex <==
\begin{table*}[ht!]
    \begin{subtable}[h]{0.49\textwidth}
        \centering
        \scriptsize
        \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}} lccccc}
        \toprule
        RICO & \multicolumn{4}{c}{Conditioned on Category} & + Size\\
        \cmidrule(lr){2-5} \cmidrule(lr){6-6}
        Model & IOU$\downarrow$ & Overlap$\downarrow$ & Alignment$\downarrow$ & Sim.$\uparrow$ & Sim.$\uparrow$ \\
        \midrule
        Trans. & 0.24{\mytiny$\pm0.2\%$}	& 0.33{\mytiny$\pm0.8\%$}	& 0.30{\mytiny$\pm0.8\%$}	 & 0.20{\mytiny$\pm0.1\%$} & -\\
        VTN &  \textbf{0.22}{\mytiny$\pm0.1\%$} & 0.30{\mytiny$\pm0.3\%$} & 0.32{\mytiny$\pm0.9\%$} & 0.20{\mytiny$\pm0.1\%$} & - \\
        Ours & \textbf{0.22}{\mytiny$\pm0.4\%$} & \textbf{0.23}{\mytiny$\pm0.2\%$} & \textbf{0.20}{\mytiny$\pm1.1\%$} & \textbf{0.21}{\mytiny$\pm0.2\%$} & \textbf{0.30}\\
        \midrule
       \end{tabular*}
       \label{tab:condi_rico}
    \end{subtable}
    \hfill
    \begin{subtable}[h]{0.49\textwidth}
        \centering
        \scriptsize
        \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}} lccccc}
        \toprule
        PubLayNet& \multicolumn{4}{c}{Conditioned on Category} & + Size\\
        \cmidrule(lr){2-5} \cmidrule(lr){6-6}
        Model & IOU$\downarrow$ & Overlap$\downarrow$ & Alignment$\downarrow$ & Sim.$\uparrow$ & Sim.$\uparrow$ \\
        \midrule
        Trans. &  \textbf{0.09}{\mytiny$\pm0.3\%$} & 0.06{\mytiny$\pm0.3\%$} & 0.33{\mytiny$\pm0.3\%$} & \textbf{0.11}{\mytiny$\pm0.1\%$} & -\\
        VTN & 0.10{\mytiny$\pm0.6\%$} & 0.06{\mytiny$\pm0.2\%$} & 0.33{\mytiny$\pm0.4\%$} & 0.10{\mytiny$\pm0.1\%$} & -\\
        Ours & \textbf{0.09}{\mytiny$\pm0.2\%$} & \textbf{0.04}{\mytiny$\pm0.1\%$} & \textbf{0.25}{\mytiny$\pm0.7\%$} & \textbf{0.11}{\mytiny$\pm0.2\%$} & \textbf{0.18} \\
        \midrule
       \end{tabular*}
       \label{tab:condi_publaynet}
    \end{subtable}
    \hfill
    \begin{subtable}[h]{0.49\textwidth}
        \centering
        \scriptsize
        \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}} lccccc}
        \toprule
        COCO & \multicolumn{4}{c}{Conditioned on Category} & + Size\\
        \cmidrule(lr){2-5} \cmidrule(lr){6-6}
        Model & IOU$\downarrow$ & Overlap$\downarrow$ & Alignment$\downarrow$ & Sim.$\uparrow$ & Sim.$\uparrow$ \\
        \midrule
        Trans.& 0.60{\mytiny$\pm0.4\%$}  & \textbf{1.66}{\mytiny$\pm2.0\%$}  & 0.34{\mytiny$\pm0.2\%$}  & 0.20{\mytiny$\pm0.2\%$}  & -\\
        VTN & 0.63{\mytiny$\pm0.4\%$}  & 1.79{\mytiny$\pm1.6\%$}  & 0.32{\mytiny$\pm0.3\%$}  & 0.22{\mytiny$\pm0.1\%$}  & -\\
        Ours & \textbf{0.35}{\mytiny$\pm0.5\%$}  & 1.93{\mytiny$\pm5.0\%$}  & \textbf{0.16}{\mytiny$\pm0.5\%$}  & \textbf{0.24}{\mytiny$\pm0.1\%$}  & \textbf{0.44}\\
        \midrule
       \end{tabular*}
       \label{tab:condi_coco}
    \end{subtable}
    \hfill
    \begin{subtable}[h]{0.49\textwidth}
        \centering
        \scriptsize
        \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}} lccccc}
        \toprule
        Magazine& \multicolumn{4}{c}{Conditioned on Category} & + Size\\
        \cmidrule(lr){2-5} \cmidrule(lr){6-6}
        Model & IOU$\downarrow$ & Overlap$\downarrow$ & Alignment$\downarrow$ & Sim.$\uparrow$ & Sim.$\uparrow$ \\
        \midrule
        Trans. & 0.20{\mytiny$\pm0.8\%$}  & 0.22{\mytiny$\pm1.6\%$}  & 0.48{\mytiny$\pm1.1\%$}  & 0.15{\mytiny$\pm0.3\%$}  & - \\
        VTN & \textbf{0.16}{\mytiny$\pm0.7\%$}  &	0.22{\mytiny$\pm3.4\%$}  & 0.47{\mytiny$\pm1.4\%$}  & 	0.15{\mytiny$\pm0.9\%$}  & -\\
        Ours & \textbf{0.16}{\mytiny$\pm0.6\%$}  & \textbf{0.12}{\mytiny$\pm0.7\%$}  & \textbf{0.44}{\mytiny$\pm2.7\%$} & \textbf{0.17}{\mytiny$\pm0.4\%$} & \textbf{0.26} \\
        \midrule
       \end{tabular*}
       \label{tab:condi_magazine}
    \end{subtable}
     \caption{Category (+ Size)  conditional  layout generation performance on various benchmarks.}
     \label{tab:cond_rst}
\end{table*}




\begin{table}
\centering
\scriptsize
\begin{tabular}{lccccc}
\toprule
Ads & \multicolumn{4}{c}{Conditioned on Category} & + Size\\
\cmidrule(lr){2-5} \cmidrule(lr){6-6}
Model & IOU$\downarrow$ & Overlap$\downarrow$ & Alignment$\downarrow$ & Sim.$\uparrow$ & Sim.$\uparrow$ \\
\midrule
Trans & 0.19{\mytiny$\pm0.1\%$}  & 0.15{\mytiny$\pm0.1\%$}  & 0.35{\mytiny$\pm0.1\%$}  & 0.30{\mytiny$\pm0.1\%$}  & - \\
VTN & 0.18{\mytiny$\pm0.2\%$}  & 0.15{\mytiny$\pm0.1\%$}  & 0.33{\mytiny$\pm0.1\%$}  & 0.31{\mytiny$\pm0.1\%$}  & - \\
Ours & \textbf{0.10}{\mytiny$\pm0.4\%$}  & \textbf{0.10}{\mytiny$\pm0.4\%$}  & \textbf{0.18}{\mytiny$\pm0.6\%$}  & \textbf{0.30}{\mytiny$\pm0.1\%$}  & 0.41 \\
\bottomrule
\end{tabular}
\caption{Conditional generation performance on Image Ads.}
\label{tab:condi_superbloom}
\end{table}


==> tables/decoding_speed.tex <==
\begin{table}[t]
\centering
\begin{tabular}{cccc}
\toprule
& Uncond. & C. Cond.\\
\midrule
Trans. & 1X & 1X \\
VTN. & 1X & 1X \\
Ours & 3.1X & 3.9X\\
\bottomrule
\end{tabular}
\caption{Decoding speed comparison of various models for different generation scenarios on RICO dataset. Uncond., C. Cond. denote unconditional, category conditional generations respectively.
}
\label{tab:decode-speed}
\end{table}


==> tables/ndn.tex <==
\begin{table}[t]
\centering
\begin{tabular}{ccc}
\toprule
Model & Magazine & RICO \\
\midrule
NDN-none (unconditional) & 2.51{\mytiny$\pm$0.09} & 0.91{\mytiny$\pm$0.03}\\
NDN-all  (conditional) & 1.51{\mytiny$\pm$0.09} & 0.32{\mytiny$\pm$0.02} \\
Ours (conditional) & \textbf{0.45}{\mytiny$\pm$0.03} & \textbf{0.25}{\mytiny$\pm$0.11}\\
\bottomrule
\end{tabular}
\caption{Comparison to the state-of-the-art conditional VAE~\cite{lee2020neural} using the metric Alignment$\downarrow$ on RICO and Magazine.
}
\label{tab:ndn}
\end{table}

